A survey of the high order multiplicity of nearby solar-type binary stars with Robo-AO

We conducted a survey of nearby binary systems composed of main sequence stars of spectral types F and G in order to improve our understanding of the hierarchical nature of multiple star systems. Using Robo-AO, the first robotic adaptive optics instrument, we collected high angular resolution images with deep and well-defined detection limits in the SDSS $i'$ band. A total of 695 components belonging to 595 systems were observed. We prioritized observations of faint secondary components with separations over $10''$ to quantify the still poorly constrained frequency of their sub-systems. Of the 214 secondaries observed, 39 contain such subsystems; 19 of those were discovered with Robo-AO. The selection-corrected frequency of secondary sub-systems with periods from $10^{3.5}$ to $10^5$ days is 0.12$\pm$0.03, the same as the frequency of such companions to the primary. Half of the secondary pairs belong to quadruple systems where the primary is also a close pair, showing that the presence of sub-systems in both components of the outer binary is correlated. The relatively large abundance of 2+2 quadruple systems is a new finding, and will require more exploration of the formation mechanism of multiple star systems. We also targeted close binaries with periods less than 100~yr, searching for their distant tertiary components, and discovered 17 certain and 2 potential new triples. In a sub-sample of 241 close binaries, 71 have additional outer companions. The overall frequency of tertiary components is not enhanced, compared to all (non-binary) targets, but in the range of outer periods from $10^6$ to $10^{7.5}$ days (separations on the order of 500~AU), the frequency of tertiary components is 0.16$\pm$0.03, exceeding by almost a factor of two the frequency of similar systems among all targets (0.09).

==> table_orbit_ephemeris.tex <==

\begin{deluxetable}{ll@{~}r@{~}lrrrrrr}
\tabletypesize{\scriptsize}
\tablewidth{0pt}
\tablecaption{Orbital Ephemerides}
\tablehead{
\colhead{WDS} & 
\multicolumn{3}{c}{Discoverer} &
\multicolumn{1}{c}{2014.0} &
\multicolumn{1}{c}{2016.0} &
\multicolumn{1}{c}{2018.0} &
\multicolumn{1}{c}{2020.0} &
\multicolumn{1}{c}{2022.0} &
\multicolumn{1}{c}{2024.0} \\
\colhead{Designation} &   
\multicolumn{3}{c}{Designation} &
\colhead{$\theta$~~~~~~~~$\rho$} & 
\colhead{$\theta$~~~~~~~~$\rho$} & 
\colhead{$\theta$~~~~~~~~$\rho$} & 
\colhead{$\theta$~~~~~~~~$\rho$} & 
\colhead{$\theta$~~~~~~~~$\rho$} & 
\colhead{$\theta$~~~~~~~~$\rho$} \\
}
\startdata
00335$+$4006 & HO  &    3 &    & 144.9~~~0.339~ & 140.3~~~0.372~ & 136.5~~~0.402~ & 133.2~~~0.427~ & 130.1~~~0.447~ & 127.4~~~0.462~ \\
01158$+$0947 & A   & 2102 &    & 110.6~~~0.265~ & 106.0~~~0.245~ & 100.6~~~0.227~ &  94.4~~~0.211~ &  87.2~~~0.197~ &  79.0~~~0.186~ \\
01417$-$1119 & STF &  147 &    & 261.2~~~0.189~ & 269.1~~~0.244~ & 276.4~~~0.209~ & 289.9~~~0.136~ & 331.7~~~0.074~ &  36.0~~~0.101~ \\
02371$-$1216 & HU  & 1216 &    &  35.1~~~0.657~ &  36.8~~~0.670~ &  38.6~~~0.683~ &  40.2~~~0.697~ &  41.8~~~0.711~ &  43.3~~~0.725~ \\
02517$+$4559 & A   & 1281 &    & 141.4~~~0.643~ & 143.4~~~0.648~ & 145.4~~~0.653~ & 147.3~~~0.656~ & 149.3~~~0.658~ & 151.2~~~0.659~ \\
03140$+$0044 & STF &  367 &    & 131.1~~~1.228~ & 130.4~~~1.237~ & 129.7~~~1.245~ & 129.0~~~1.253~ & 128.3~~~1.261~ & 127.6~~~1.268~ \\
03413$+$4554 & BU  & 1181 & AB &  87.4~~~0.041~ & 285.1~~~0.006~ & 271.1~~~0.050~ & 270.1~~~0.075~ &  90.3~~~0.056~ &  90.0~~~0.174~ \\
03496$-$0220 & YR  &   23 &    & 308.0~~~0.353~ & 301.4~~~0.372~ & 295.5~~~0.391~ & 290.1~~~0.410~ & 285.2~~~0.429~ & 280.7~~~0.446~ \\
04163$+$0710 & WSI &   97 &    & 131.6~~~0.171~ & 157.3~~~0.146~ & 287.8~~~0.091~ & 324.1~~~0.209~ & 343.7~~~0.174~ &  47.4~~~0.080~ \\
04422$+$3731 & STF &  577 &    & 333.8~~~0.702~ & 329.6~~~0.687~ & 325.3~~~0.674~ & 320.8~~~0.663~ & 316.1~~~0.655~ & 311.4~~~0.648~ \\
07043$-$0303 & A   &  519 & AB & 103.4~~~0.111~ &  86.0~~~0.059~ & 297.5~~~0.070~ & 286.1~~~0.171~ & 282.8~~~0.247~ & 280.9~~~0.303~ \\
07092$+$1903 & CHR &  216 &    & 162.1~~~0.134~ & 158.7~~~0.167~ & 156.3~~~0.196~ & 154.6~~~0.220~ & 153.1~~~0.240~ & 151.9~~~0.256~ \\
08122$+$1739 & HUT & 1 & Ca,Cb &   3.7~~~0.343~ & 324.0~~~0.336~ & 285.6~~~0.348~ & 248.2~~~0.339~ & 204.9~~~0.306~ & 155.5~~~0.309~ \\
08531$+$5457 & A   & 1584 &    &  90.2~~~0.671~ &  92.5~~~0.675~ &  94.8~~~0.675~ &  97.1~~~0.673~ &  99.5~~~0.667~ & 101.8~~~0.659~ \\
10387$+$0544 & STF & 1457 &    & 333.5~~~1.840~ & 333.7~~~1.841~ & 333.9~~~1.842~ & 334.1~~~1.843~ & 334.3~~~1.844~ & 334.5~~~1.844~ \\
11293$+$3025 & L   &   11 &    & 281.8~~~1.025~ & 280.5~~~1.026~ & 279.2~~~1.027~ & 277.9~~~1.027~ & 276.7~~~1.026~ & 275.4~~~1.024~ \\
13577$+$5200 & A   & 1614 &    & 120.3~~~1.393~ & 119.6~~~1.397~ & 118.9~~~1.400~ & 118.2~~~1.402~ & 117.5~~~1.403~ & 116.8~~~1.403~ \\
14525$+$1844 & BU  &   31 & AB & 220.8~~~2.009~ & 221.1~~~2.011~ & 221.5~~~2.013~ & 221.9~~~2.014~ & 222.2~~~2.016~ & 222.6~~~2.017~ \\
15413$+$5959 & STF & 1969 &    &  28.8~~~1.033~ &  29.0~~~1.058~ &  29.2~~~1.083~ &  29.4~~~1.107~ &  29.6~~~1.130~ &  29.8~~~1.153~ \\
17207$-$0706 & A   & 2593 & AB & 345.5~~~0.273~ & 340.2~~~0.270~ & 334.7~~~0.261~ & 328.7~~~0.248~ & 321.9~~~0.231~ & 313.9~~~0.212~ \\
18154$+$5720 & HDS & 2577 &    & 305.9~~~0.239~ & 317.2~~~0.226~ & 329.6~~~0.220~ & 342.3~~~0.220~ & 354.7~~~0.227~ &   5.9~~~0.241~ \\
20514$-$0538 & STF & 2729 & AB &  28.7~~~0.788~ &  30.3~~~0.766~ &  31.9~~~0.744~ &  33.6~~~0.722~ &  35.4~~~0.699~ &  37.3~~~0.677~ \\
21041$+$0300 & WSI &    6 & AB & 278.0~~~0.266~ & 287.5~~~0.277~ & 297.9~~~0.245~ & 314.0~~~0.179~ & 351.9~~~0.110~ &  57.2~~~0.119~ \\
21243$+$3740 & WSI &    7 &    & 355.2~~~0.065~ & 259.6~~~0.119~ & 230.2~~~0.148~ & 200.9~~~0.128~ & 160.5~~~0.114~ & 121.7~~~0.134~ \\
\enddata
\end{deluxetable}

